Justificatory and Explanatory Argumentation for Committing Agents

In the interaction between agents we can have an explicative discourse, when communicating preferences or intentions, and a normative discourse, when considering normative knowledge. For justifying their actions our agents are endowed with a Justification and Explanation Logic (JEL), capable to cover both the justification for their commitments and explanations why they had to act in that way, due to the current situation in the environment. Social commitments are used to formalise justificatory and explanatory patterns. The combination of ex- planation, justification, and commitments

==> graphs_config.tex <==
% Local configuration for version 1.53 of graphs.sty. Frank Drewes, 16.11 2003

% The \special macro below must contain the path under which the file
% graphs.header can be found in you local installation. Please modify it
% accordingly.

\special{header=./graphs.header}

